Observations of the Isotropic Diffuse Gamma-ray Background with the EGRET Telescope

An Isotropic Diffuse Gamma-Ray Background (IDGRB) in the spectral range 30-10,000 MeV was first reported in the early 1970's using measurements made by the SAS-2 instrument. Data recorded by the Energetic Gamma Ray Experiment Telescope (EGRET) on board the Compton Gamma Ray Observatory (CGRO) over the last 4 years are analysed in order to extract the best measurement yet made of the IDGRB. Extensive analysis of the EGRET instrumental background is presented in order to demonstrate that an uncontaminated data set can be extracted from the EGRET data. A model of the high latitude galactic diffuse foreground emission is presented and the existence of an IDGRB is confirmed. Spatial and spectral analysis of this background is presented. In addition, point source analysis at high galactic latitudes is performed to reveal the existence of a population of extragalactic sources. The characteristics of this population are examined and models of its flux distribution are reported. The question of whether the IDGRB is composed of unresolved point sources is addressed using fluctuation analysis. Finally, possible future directions for gamma ray astronomy are examined through simulations of a future gamma ray telescope: the Gamma-ray Large Area Space Telescope (GLAST). The GLAST baseline design is described and its scientific performance is evaluated. The ability of this telescope to detect 1,000-10,000 new extragalactic sources is demonstrated and the likely impact on the study of the IDGRB is considered.

==> Tables/error_boxes.tex <==
\centering
\caption
{Summary of 95\% Eror Contours}
\bigskip
\small
\begin{tabular}{l|cccc}\hline\hline
& \multicolumn{2}{c}{2EG J2227+6122}  \\
\cline{2-5}
Zenith Angle range & $\alpha<50.0$      & $50.0<\alpha<65.0$   & $65.0<\alpha<80.0$ & $80.0<\alpha<95.375$        \\
\hline
Fractional Exposure            & 0.38      & 0.24   & 0.24 & 0.14         \\[0.1in]
Differential Albedo            & 0.0      & $0.4 \pm 0.4$   & $1.9 \pm 0.4$ & $6.8 \pm 0.6 $    \\
Intensity ($\times 10^{-6}$)& & & &   \\[0.1in]
Mean Albedo Intensity           & 0.0      & $0.15 \pm 0.15$   & $0.64 \pm 0.2$ & $1.5 \pm 0.2 $    \\
 ($\alpha<\alpha_{max}$)($\times 10^{-6}$)& & & &   \\[0.1in]
Signal:Noise           & N/A      & 66   & 16 & 7    \\[0.1in]
\hline
\hline
& \multicolumn{4}{c}{$E>1000 MeV$}  \\
\cline{2-5}
Zenith Angle range & $\alpha<65.0$      & $65.0<\alpha<80.0$   & $80.0<\alpha<95.0$ & $95.0<\alpha<105$        \\
\hline
Fractional Exposure            &   .60  &  .25  & .13 &    .02      \\[0.1in]
Differential Albedo            &   0    &  $-1.5 \pm 1.0$ & $3.4 \pm 1.5$ &  $48.8 \pm 6.5$   \\[0.1in]
Intensity ($\times 10^{-7}$)& & & &   \\[0.1in]
Mean Albedo Intensity           & 0.0      & $0.0 \pm 0.3$   & $0.45 \pm 0.32$ & $1.41 \pm 0.3 $    \\
 ($\alpha<\alpha_{max}$)($\times 10^{-6}$)& & & &   \\[0.1in]
Signal:Noise           & N/A      & $>33$   & 22 & 7    \\[0.1in]
\hline
\hline
\end{tabular}


==> Tables/zencuts.tex <==
\centering
\caption
{Summary of Albedo Contamination Investigation Results}
\bigskip
\small
\begin{tabular}{l|cccc}\hline\hline
& \multicolumn{4}{c}{$E>100 MeV$}  \\
\cline{2-5}
Zenith Angle range & $\alpha<50.0$      & $50.0<\alpha<65.0$   & $65.0<\alpha<80.0$ & $80.0<\alpha<95.375$        \\
\hline
Fractional Exposure            & 0.38      & 0.24   & 0.24 & 0.14         \\[0.1in]
Albedo Intensity            & 0.0      & $0.4 \pm 0.4$   & $1.9 \pm 0.4$ & $6.8 \pm 0.6 $    \\[0.1in]
($\times 10^{-6}$)& & & &   \\
\hline
\hline
& \multicolumn{4}{c}{$E>1000 MeV$}  \\
\cline{2-5}
Zenith Angle range & $\alpha<65.0$      & $65.0<\alpha<80.0$   & $80.0<\alpha<95.0$ & $95.0<\alpha<105$        \\
\hline
Fractional Exposure            & 0.25      & 0.25   & 0.25 & 0.25         \\[0.1in]
Albedo Intensity            & 0.0      & $0.5 \pm 0.4$   & $1.9 \pm 0.6$ & $6.8 \pm 0.6 $    \\[0.1in]
($\times 10^{-7}$)& & & &   \\
\hline
\hline
\end{tabular}

